Domain Representative Keywords Selection: A Probabilistic Approach

We propose a probabilistic approach to select a subset of a \textit{target domain representative keywords} from a candidate set, contrasting with a context domain. Such a task is crucial for many downstream tasks in natural language processing. To contrast the target domain and the context domain, we adapt the \textit{two-component mixture model} concept to generate a distribution of candidate keywords. It provides more importance to the \textit{distinctive} keywords of the target domain than common keywords contrasting with the context domain. To support the \textit{representativeness} of the selected keywords towards the target domain, we introduce an \textit{optimization algorithm} for selecting the subset from the generated candidate distribution. We have shown that the optimization algorithm can be efficiently implemented with a near-optimal approximation guarantee. Finally, extensive experiments on multiple domains demonstrate the superiority of our approach over other baselines for the tasks of keyword summary generation and trending keywords selection.

==> tables/newsgroup_classification.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{@{}llllllll@{}}
\toprule
$k$   & \multicolumn{1}{c}{RF}      & \multicolumn{1}{c}{LO}      & \multicolumn{1}{c}{PR}      & \multicolumn{1}{c}{FL}      &  \multicolumn{1}{c}{$\mathbf{KL_{rf}}$} & \multicolumn{1}{c}{MM}               & \multicolumn{1}{c}{$\mathbf{KL_{mm}}$}                     \\ \midrule
10   & \textbf{0.5676} $\pm$ 0.01 & 0.4879 $\pm$ 0.01 & 0.5644 $\pm$ 0.01  & 0.5115 $\pm$ 0.01 & \textbf{0.5676} $\pm$ 0.01 & 0.5244 $\pm$ 0.02 & 0.5451 $\pm$ 0.01 \\
20   & 0.6249 $\pm$ 0.01 & 0.5664 $\pm$ 0.02 & 0.6232 $\pm$ 0.01  & 0.556 $\pm$ 0.02  & 0.6425 $\pm$ 0.01 & 0.6088 $\pm$ 0.01 & \textbf{0.6465} $\pm$ 0.01 \\
30   & 0.686 $\pm$ 0.01  & 0.6034 $\pm$ 0.02 & 0.6803 $\pm$ 0.01  & 0.5955 $\pm$ 0.01 & 0.6844 $\pm$ 0.01 & 0.6845 $\pm$ 0.01 & \textbf{0.6941} $\pm$ 0.01 \\
40   & 0.7042 $\pm$ 0.01 & 0.6243 $\pm$ 0.02 & 0.6974 $\pm$ 0.01 & 0.6446 $\pm$ 0.02 & 0.7181 $\pm$ 0.01 & 0.6929 $\pm$ 0.01 & \textbf{0.7159} $\pm$ 0.01 \\
50   & 0.7298 $\pm$ 0.01 & 0.6583 $\pm$ 0.01 & 0.7099 $\pm$ 0.01  & 0.6785 $\pm$ 0.01 & 0.7308 $\pm$ 0.01 & \textbf{0.7362} $\pm$ 0.01 & 0.7335 $\pm$ 0.01 \\
100  & 0.7743 $\pm$ 0.01 & 0.7105 $\pm$ 0.01 & 0.755 $\pm$ 0.01   & 0.7456 $\pm$ 0.01 & 0.778 $\pm$ 0.01  & 0.773 $\pm$ 0.01  & \textbf{0.7781} $\pm$ 0.01 \\
200  & 0.8216 $\pm$ 0.01 & 0.7749 $\pm$ 0.01 & 0.8126 $\pm$ 0.01  & 0.7855 $\pm$ 0.01 & 0.8234 $\pm$ 0.01 & 0.8195 $\pm$ 0.01 & \textbf{0.8239} $\pm$ 0.01 \\
300  & 0.8399 $\pm$ 0.02 & 0.8143 $\pm$ 0.01 & 0.8371 $\pm$ 0.01  & 0.8211 $\pm$ 0.01 & 0.8434 $\pm$ 0.01 & 0.8471 $\pm$ 0.01 & \textbf{0.8512} $\pm$ 0.01 \\
400  & 0.855 $\pm$ 0.01  & 0.8245 $\pm$ 0.01 & 0.8475 $\pm$ 0.01  & 0.8401 $\pm$ 0.01 & \textbf{0.8612} $\pm$ 0.01 & 0.8592 $\pm$ 0.01 & 0.8581 $\pm$ 0.01 \\
500  & 0.8690 $\pm$ 0.01  & 0.8359 $\pm$ 0.01 & 0.8577 $\pm$ 0.01  & 0.8464 $\pm$ 0.01 & \textbf{0.8697} $\pm$ 0.01 & 0.865 $\pm$ 0.01  & 0.8669 $\pm$ 0.01 \\
1000 & 0.8843 $\pm$ 0.01 & 0.8675 $\pm$ 0.01 & 0.8779 $\pm$ 0.01  & 0.8688 $\pm$ 0.01 & \textbf{0.8856} $\pm$ 0.01 & 0.8809 $\pm$ 0.01 & 0.8827 $\pm$ 0.01 \\
2000 & \textbf{0.8993} $\pm$ 0.01 & 0.8829 $\pm$ 0.01 & 0.8969 $\pm$ 0.01  & 0.888 $\pm$ 0.01  & 0.8984 $\pm$ 0.01 & \textbf{0.8993} $\pm$ 0.01 & 0.8985 $\pm$ 0.01 \\ \bottomrule
\end{tabular}}
\end{table*}

==> tables/temporal_summary_additional.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[!htbp]
\scriptsize
% \footnotesize
\centering
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{p{0.05\textwidth}p{0.3\textwidth}p{0.3\textwidth}p{0.3\textwidth}}
\toprule
                                                          & \multicolumn{1}{c}{2000-2009}                                                                                                                                                                                                                                                                                                             & \multicolumn{1}{c}{2010-2019}                                                                                                                                                                                                                                                                                                                             & \multicolumn{1}{c}{2020-2021}                                                                                                                                                                                                                                                                                    \\ \midrule
RF                                                         & paper, problem, \textbf{algorithm}, model, method, approach, \textbf{system},   information, result, datum, set, application, number, user, word,   performance, language, order, time, case                                                                                                                                                                & model, method, paper, approach, image, problem, datum, task,   algorithm, dataset, performance, network, result, feature, system, training,   application, work, number, object                                                                                                                                                       & model, method, task, datum, approach, dataset, image, paper,   performance, problem, training, algorithm, network, feature, result, system,   work, \textbf{application}, \textbf{deep learning}, experiment                                                                                                                                                                                    \\ \midrule
FL                                                         & paper, problem, \textbf{algorithm}, model, method, approach, \textbf{system},   result, information, set, application, datum, number, user, word, order,   performance, case, image, time                                                                                                                                                                   & image, model, method, paper, problem, approach, datum,   algorithm, task, network, performance, dataset, result, user, application,   work, feature, system, training, number                                                                                                                                                         & image, model, method, paper, task, datum, approach, dataset,   performance, problem, training, algorithm, work, result, network, experiment,   \textbf{application}, system, feature, \textbf{deep learning}                                                                                                                       \\ \midrule
{$\mathbf{KL_{mm}}$}     & problem, paper, \textbf{algorithm}, method, model, \textbf{system}, approach,   information, datum, word, set, result, user, application, \textbf{agent}, number,   network, performance, \textbf{language}, order                                                                                                                                                            & image, model, method, algorithm, datum, paper, task, network,   problem, approach, dataset, system, user, feature, performance, training,   object, application, result, information                                                                                                                                                  & model, method, image, task, datum, dataset, problem, network,   approach, paper, training, algorithm, system, performance, feature, object,   \textbf{application}, user, \textbf{deep learning}, result                                                                                                     \\ \bottomrule
\end{tabular}}
{\raggedright \centering Keywords representative of its corresponding time frame are \textbf{highlighted} (annotated by authors). \par}
% \vspace{-3mm}
\caption{Keyword summaries (top 20 keywords) of three different time frames in AI domain}
\label{tab:time_summ_rest}
% \vspace{-5mm}
\end{table*}

==> tables/temporal_summary_mainpart.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[!hbt]
\scriptsize
% \footnotesize
\centering
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{p{0.04\textwidth}p{0.35\textwidth}p{0.35\textwidth}p{0.35\textwidth}}
\toprule
                                                          & \multicolumn{1}{c}{2000-2009}                                                                                                                                                                                                                                                                                                             & \multicolumn{1}{c}{2010-2019}                                                                                                                                                                                                                                                                                                                             & \multicolumn{1}{c}{2020-2021}                                                                                                                                                                                                                                                                                    \\ \midrule

LO                                                         & \textbf{logic program}, rule, manipulator, \textbf{genetic algorithm},   workspace, \textbf{parallel manipulator}, \textbf{logic programming}, document, grammar, stable   model, \textbf{artificial immune system}, logic, word, web site, \textbf{answer set}, global   constraint, \textbf{machining}, fitness, belief, evolvability                                                                  & image, dataset, method, feature, task, \textbf{convolutional neural network}, object, training, \textbf{deep learning}, classification, classifier, \textbf{deep   neural network}, \textbf{neural network}, robot, model, video, \textbf{recurrent neural   network}, word, \textbf{segmentation}, representation                                                                        & model, dataset, task, training, \textbf{transformer}, image, \textbf{deep   learning}, \textbf{neural network}, prediction, label, \textbf{federated learning}, learning,   method, \textbf{machine learning}, \textbf{language model}, explanation, experiment, \textbf{covid 19},   \textbf{reinforcement learning}, feature                                                           \\\midrule
PR                                                         & problem, \textbf{algorithm}, paper, user, datum, model, word, method,   image, information, approach, \textbf{system}, constraint, set, solution, performance,   application, document, result, rule                                                                                                                                                        & image, algorithm, user, robot, object, network, word, model,   dataset, agent, environment, datum, task, video, method, training, \textbf{language},   system, policy, \textbf{segmentation}                                                                                                                                                            & image, robot, model, object, algorithm, dataset, task, agent,   environment, user, datum, policy, language, graph, \textbf{reinforcement learning},   network, method, video, training, \textbf{deep learning}                                                                                                                    \\ \midrule
MM                                                         & \textbf{logic program}, manipulator, \textbf{genetic algorithm}, workspace,   \textbf{parallel manipulator}, \textbf{logic programming}, grammar, \textbf{stable model}, \textbf{artificial   immune system}, web site, \textbf{answer set}, \textbf{global constraint}, \textbf{machining}, fitness,   \textbf{evolvability}, \textbf{radial distortion}, \textbf{soft constraint}, \textbf{nonmonotonic reasoning},   \textbf{stable model semantic}, \textbf{belief revision} & image, \textbf{convolutional neural network}, \textbf{recurrent neural network},   classifier, \textbf{deep convolutional neural network}, \textbf{deep network}, \textbf{cnn}, \textbf{computer   vision}, \textbf{lstm}, \textbf{deep neural network}, \textbf{bayesian network}, \textbf{rnn}, \textbf{word embedding},   \textbf{svm}, \textbf{segmentation}, \textbf{convolutional network}, \textbf{descriptor}, \textbf{neural machine   translation}, recognition, sentence   & \textbf{transformer}, training, \textbf{federated learning}, \textbf{language model},   \textbf{covid 19}, \textbf{graph neural network}, dataset, explanation, \textbf{deep learning}, \textbf{pre   training}, \textbf{adversarial attack}, \textbf{fine tuning}, \textbf{meta learning}, \textbf{deep learning}   model, lidar, \textbf{self attention}, point cloud, \textbf{reinforcement learning}, \textbf{bert},   label               \\ \midrule
{$\mathbf{KL_{mm}}$} & \textbf{
logic program}, workspace, \textbf{genetic algorithm}, grammar,   manipulator, \textbf{logic programming}, web site, \textbf{global constraint}, \textbf{artificial   immune system}, \textbf{evolvability}, \textbf{parallel manipulator}, synonym, \textbf{stable model},   \textbf{som}, \textbf{belief revision}, \textbf{unification}, \textbf{soft constraint}, \textbf{language resource}, fitness,   \textbf{wordnet}                                          & image, \textbf{convolutional neural network}, \textbf{recurrent neural network},   classifier, \textbf{deep network}, \textbf{deep convolutional neural network}, \textbf{bayesian   network}, \textbf{word embedding}, \textbf{computer vision}, \textbf{descriptor}, \textbf{svm}, \textbf{crf}, \textbf{lstm}, \textbf{neural   machine translation}, dictionary, \textbf{convolutional network}, \textbf{deep neural network},   \textbf{recognition}, \textbf{cnn}, \textbf{segmentation} & \textbf{transformer}, training, explanation, \textbf{language model}, \textbf{covid 19},   \textbf{federated learning}, \textbf{graph neural network}, dataset, \textbf{pre training}, lidar, \textbf{deep   learning}, \textbf{adversarial attack}, label, \textbf{meta learning}, \textbf{knowledge distillation},   \textbf{fine tuning}, \textbf{deep learning model}, \textbf{latent space}, \textbf{datum augmentation}, \textbf{target   domain} \\ \bottomrule
\end{tabular}}
{\raggedright \centering Keywords representative of its corresponding time frame are \textbf{highlighted} (annotated by authors). \par}
\vspace{-2mm}
\caption{Keyword summaries (top 20 keywords) of three different time frames in AI domain}
\label{tab:time_summ}
\vspace{-3mm}
\end{table*}
